Effect of the atomic structure of complexions on the active disconnection mode during shear-coupled grain boundary motion

The migration of grain boundaries leads to grain growth in polycrystals and is one mechanism of grain-boundary-mediated plasticity, especially in nanocrystalline metals. This migration is due to the movement of dislocation-like defects, called disconnections, which couple to externally applied shear stresses. While this has been studied in detail in recent years, the active disconnection mode was typically associated with specific macroscopic grain boundary parameters. We know, however, that varying microscopic degrees of freedom can lead to different atomic structures without changing the macroscopic parameters. These structures can transition into each other and are called complexions. Here, we investigate $[11\overline{1}]$ symmetric tilt boundaries in fcc metals, where two complexions -- dubbed domino and pearl -- were observed before. We compare these two complexions for two different misorientations: In $\Sigma19$b $[11\overline{1}]$ $(178)$ boundaries, both complexions exhibit the same disconnection mode. The critical stress for nucleation and propagation of disconnections is nevertheless different for domino and pearl. At low temperatures, the Peierls-like barrier for disconnection propagation dominates, while at higher temperatures the nucleation is the limiting factor. For $\Sigma$7 $[11\overline{1}]$ $(145)$ boundaries, we observed a larger difference. The domino and pearl complexions migrate in different directions under the same boundary conditions. While both migration directions are possible crystallographically, an analysis of the complexions' structural motifs and the disconnection core structures reveals that the choice of disconnection mode and therefore migration direction is directly due to the atomic structure of the grain boundary.

==> convert <==
#!/usr/bin/env python3

import os
import re
import io
import subprocess
import shutil
import tempfile

# Check these settings!
TEX_NAME = "../main.tex"
OUT_NAME = "paper.tex"
CONV_PDF_TO_EPS = False  # convert .pdf to .eps?
EMBED_BIBTEX = True      # paste the .bbl file into the .tex?
SHRINK_PDF = False       # use ghostscript to reduce the resolution of
                         # PDF images; set to False to disable and to
                         # an integer to scale to this dpi
SHRINK_THRESHOLD = 1024  # kB; only try to shrink files bigger than this

# Command to convert to .eps
PDF2EPS_CMD = ["pdftops", "-eps", "-level3"]

# Command to shrink PDFs.
GS_CMD = ["gs", "-dNOPAUSE", "-dQUIET", "-dBATCH", "-dSAFER",
          "-sDEVICE=pdfwrite", "-dPDFSETTINGS=/printer",
          "-dCompatibilityLevel=1.5",
          "-dEmbedAllFonts=true", "-dSubsetFonts=true",
          "-dAutoRotatePages=/None",
          "-dColorImageResolution={}".format(SHRINK_PDF),
          "-dGrayImageResolution={}".format(SHRINK_PDF),
          "-dMonoImageResolution={}".format(SHRINK_PDF),
          "-sOutputFile={outfile}", "{infile}"]


########################################################################

# Derived globals.
RELPATH = os.path.dirname(TEX_NAME)


# Helper functions #####################################################
def get_bbl(tex_name=TEX_NAME):
    bbl_path = tex_name.rsplit(".", 1)[0] + ".bbl"
    with open(bbl_path) as f:
        return f.read()


def pdf2eps(infile, outfile):
    subprocess.run(PDF2EPS_CMD + [infile, outfile], check=True)


def shrink_pdf(infile, outfile):
    if os.path.getsize(infile) // 1024 < SHRINK_THRESHOLD:
        shutil.copy(infile, outfile)
    else:
        cmdline = [token.format(infile=infile, outfile=outfile)
                   for token in GS_CMD]
        subprocess.run(cmdline, check=True)


# Parse the .tex file ##################################################
class Token:
    def __init__(self, value, is_cmd):
        self.value = value
        self.is_cmd = is_cmd

    def __str__(self):
        return self.value


def strip_comments(tex_in, comment_cre=re.compile(r'(?<!\\)(?:\\\\)*%')):
    """Remove comments from tex_in."""
    tex_out = ""
    for line in io.StringIO(tex_in):
        m = comment_cre.search(line)
        if m:
            clean_line = line[:m.end()] # leave the comment sign itself in,
                                        # it may be significant!
            clean_line = clean_line.rstrip("\n") + "\n"
        else:
            clean_line = line
        tex_out += clean_line
    return tex_out


def tokenize(tex_in):
    """Tokenize a TeX string."""
    # First, split at commands (\foo), taking into account that a
    # command may be preceeded by a newline (\\\foo)! The newlines are
    # included with the command token in this step.
    l = re.split(r'((?<!\\)(?:\\\\)*\\[a-zA-Z]+)', tex_in)
    # Move newlines out of command tokens.
    l2 = []
    for i, token in enumerate(l):
        if i % 2 == 0:
            # Not a command.
            l2.append(Token(token, False))
        else:
            # Is a command, split out newlines if necessary.
            idx = token.rfind('\\')
            if idx > 0:
                # There were one or more newline commands.
                l2.append(Token(token[:idx], False))
            l2.append(Token(token[idx:], True))
    l = l2
    del l2
    return l


figure_cre = re.compile(r'\s*\{\s*(?:figure|extfig)\s*\*?\s*\}')
def parse_and_replace_and_write(tokens, out_name=OUT_NAME):
    """Search the images for the figures and the bibliography and replace."""
    with open(out_name, "w") as tex_out:
        state = "text"
        bbl = None
        current_cmd = None # just for error messages
        fig_num = 0
        subfig_num = 0
        for token in tokens:
            if state == "text":
                if not token.is_cmd:
                    tex_out.write(token.value)
                else:
                    # Check if it is a command we care about.
                    if token.value == r'\bibliography' and EMBED_BIBTEX:
                        state = "remove-arg"       # need to remove the
                        current_cmd = token.value  # argument, too
                        if bbl is None:
                            bbl = get_bbl()
                        else:
                            print("WARNING: At least two bibliographies found!")
                            print("         The results may not be correct!")
                        tex_out.write(bbl)
                        tex_out.write("\n") # ensure newline!
                    elif token.value == r'\bibliographystyle' and EMBED_BIBTEX:
                        state = "remove-arg"       # need to remove the
                        current_cmd = token.value  # argument, too
                        # Write nothing, just remove the command.
                    elif token.value == r'\begin':
                        # We need to check if we are in a figure env.
                        state = "begin-env"
                        tex_out.write(token.value)
                    else:
                        tex_out.write(token.value)
            elif state == "remove-arg":
                curlybrace_count = 0
                for i, char in enumerate(token.value):
                    if char == "{":
                        curlybrace_count += 1
                    elif char == "}":
                        curlybrace_count -= 1
                        if curlybrace_count < 0:
                            print("WARNING: invalid TeX, close } without "
                                  "opening { after \bibliography! Check the "
                                  "output manually!")
                            tex_out.write(token.value)
                            state = "text"
                            current_cmd = None
                            break
                        elif curlybrace_count == 0:
                            # OK, we have the full argument, append
                            # the rest to outfile.
                            tex_out.write(token.value[i+1:])
                            state = "text"
                            current_cmd = None
                            break
            elif state == "begin-env":
                if figure_cre.match(token.value):
                    state = "in-figure"
                    fig_num += 1
                    subfig_num = 0
                else:
                    state = "text" # some uninteresting env.
                tex_out.write(token.value)
            elif state == "in-figure":
                if token.is_cmd:
                    # Check if we find either includegraphics or end figure.
                    if token.value == r'\end':
                        state = "end-figure"
                    elif token.value == r'\includegraphics':
                        state = "includegraphics"
                        bracket_count = 0
                tex_out.write(token.value)
            elif state == "end-figure":
                if figure_cre.match(token.value):
                    # Figure ended.
                    state = "text"
                tex_out.write(token.value)
            elif state == "includegraphics":
                # Iterate over the optional arguments.
                if bracket_count >= 0:
                    idx = -1
                    for i, char in enumerate(token.value):
                        if bracket_count == 0 and char == "{":
                            # No optional argument or optional arg over
                            bracket_count = -1
                            idx = i
                            break
                        elif char == "[":
                            bracket_count += 1
                        elif char == "]":
                            bracket_count -= 1
                            if bracket_count < 0:
                                print("WARNING: cannot parse "
                                      "\\includegraphics! Check manually!")
                                idx = -2 # error
                                break
                        elif bracket_count == 0 and not char.isspace():
                            # Hmmm, unparsable \includegraphics!
                            print("WARNING: cannot parse \\includegraphics! "
                                  " Check output!")
                            idx = -2 # error
                            break
                if idx == -2:
                    # Error, write this \includegraphics verbatim :-(
                    state = "in-figure"
                    tex_out.write(token.value)
                elif idx == -1:
                    # Have not yet found the opening curly brace.
                    tex_out.write(token.value)
                else:
                    # Write stuff until now.
                    idx += 1 # include opening brace
                    tex_out.write(token.value[:idx])
                    # Search closing brace.
                    idx2 = -1
                    for i, char in enumerate(token.value[idx:]):
                        if char == "}":
                            idx2 = i
                            break
                    if idx2 < 0:
                        print("WARNING: could not parse argument to "
                              "\\includegraphics. Check output!")
                        print(token.value[:idx])
                        print(token.value[idx:])
                        print()
                        tex_out.write(token.value[idx:])
                        state = "in-figure"
                    else:
                        fname = token.value[idx:idx+idx2]
                        # Get path.
                        fig_in = os.path.join(RELPATH,
                                              fname)
                        # Shrink PDF if requested.
                        if fname.endswith(".pdf") and SHRINK_PDF:
                            tmpdir = tempfile.TemporaryDirectory()
                            fig_tmp = os.path.join(tmpdir.name, "shrunk.pdf")
                            shrink_pdf(fig_in, fig_tmp)
                            fig_in = fig_tmp
                        # Convert.
                        if fname.endswith(".pdf") and CONV_PDF_TO_EPS:
                            fig_out = "fig{:02d}{}.eps".format(
                                fig_num,
                                (""
                                 if subfig_num == 0
                                 else chr(ord("a") + subfig_num))
                            )
                            pdf2eps(fig_in, fig_out)
                        else:
                            # Unknown file format or conversion not
                            # requested: use as is.
                            ending = fname.rsplit(".", 1)[-1]
                            fig_out = "fig{:02d}{}.{}".format(
                                fig_num,
                                (""
                                 if subfig_num == 0
                                 else chr(ord("a") + subfig_num)),
                                ending
                            )
                            # Copy.
                            shutil.copy(fig_in, fig_out)
                        # Clean up tmp files.
                        if fname.endswith(".pdf") and SHRINK_PDF:
                            tmpdir.cleanup()
                        # ...and output.
                        tex_out.write(fig_out)
                        tex_out.write(token.value[idx+idx2:])
                        state = "in-figure"
                        subfig_num += 1
            else:
                raise RuntimeError("State machine stuck in unknown "
                                   "state '{}', this "
                                   "is a bug, sorry".format(state))


if __name__ == "__main__":
    with open(TEX_NAME) as f:
        parse_and_replace_and_write(tokenize(strip_comments(f.read())))

